High-order accurate well-balanced energy stable adaptive moving mesh finite difference schemes for the shallow water equations with non-flat bottom topography

This paper proposes high-order accurate well-balanced (WB) energy stable (ES) adaptive moving mesh finite difference schemes for the shallow water equations (SWEs) with non-flat bottom topography. To enable the construction of the ES schemes on moving meshes, a reformulation of the SWEs is introduced, with the bottom topography as an additional conservative variable that evolves in time. The corresponding energy inequality is derived based on a modified energy function, then the reformulated SWEs and energy inequality are transformed into curvilinear coordinates. A two-point energy conservative (EC) flux is constructed, and high-order EC schemes based on such a flux are proved to be WB that they preserve the lake at rest. Then high-order ES schemes are derived by adding suitable dissipation terms to the EC schemes, which are newly designed to maintain the WB and ES properties simultaneously. The adaptive moving mesh strategy is performed by iteratively solving the Euler-Lagrangian equations of a mesh adaptation functional. The fully-discrete schemes are obtained by using the explicit strong-stability preserving third-order Runge-Kutta method. Several numerical tests are conducted to validate the accuracy, WB and ES properties, shock-capturing ability, and high efficiency of the schemes.

==> MovingMesh.tex <==
\section{Adaptive moving mesh strategy}\label{section:MM}
This section presents the adaptive moving mesh strategy that determines the mesh velocities involved in the temporal mesh metrics in \eqref{eq:Grid_Matrix_Coeff},
see \cite{DUAN2021109949,Duan2022High,Tang2003Adaptive} for more details.
Define the following mesh adaptation functional
\begin{equation*}
  \widetilde{E}(\bm{x})=\frac{1}{2} \sum_{\ell=1}^2 \int_{\Omega_c}\left(\nabla_{\bm{\xi}} x_\ell\right)^{\mathrm{T}} \bm{G}_\ell\left(\nabla_{\bm{\xi}} x_\ell\right) \mathrm{d} \bm{\xi},
\end{equation*}
and calculate its Euler-Lagrange equations
\begin{equation}\label{eq:Mesh_Control}
  \nabla_{\bm{\xi}} \cdot\left(\bm{G}_\ell \nabla_{\bm{\xi}} x_\ell\right)=0, ~\bm{\xi} \in \Omega_c, ~\ell=1,2,
\end{equation}
where $\nabla_{\bm{\xi}}$ denotes the spatial gradient in the computational domain.
Then the new redistributed mesh $\bm{x}$ in the physical domain $\Omega_p$ can be obtained by solving \eqref{eq:Mesh_Control} for a given symmetric positive definite matrix $\bm{G}_{\ell}$,
which controls the mesh concentration.
The choice of $\bm{G}_{\ell}$ is one of the most important parts of the adaptive moving mesh method,
and usually depends on the solutions of the underlying governing equations or their derivatives.
Referring to the variable diffusion method in \cite{Winslow1967Numerical}, the simplest choice is the isotropic one as follows
\begin{equation*}
  \bm{G}_\ell=\omega \bm{I}_2, ~\ell=1,2,
\end{equation*}
where the positive scalar $\omega$ is called the monitor function and this work considers
\begin{align}\label{eq:monitor}
  \omega=\Big({1+\sum_{k=1}^\kappa\theta_k\Big(
        \dfrac{\abs{\nabla_{\bm{\xi}}\sigma_k}}
  {\max\abs{\nabla_{\bm{\xi}}\sigma_k}}\Big)^2}\Big)^{1/2}.
%\omega=\sqrt{1+\alpha{\abs{\nabla_{\bm{\xi}}\sigma}}/{\max\abs{\nabla_{\bm{\xi}}\sigma}}},\nonumber
\end{align}
Here we choose $\kappa$ physical variables $\sigma_k$, and $\theta_k$ is a positive coefficient.
The monitor function \eqref{eq:monitor} is approximated by using the 2nd-order central difference for the derivatives in the computational domain,
and it is further smoothed by performing $5\sim10$ times the following low-pass filter
\begin{equation*}
  \omega_{i,j} = \sum_{i_1,j_1 = 0,\pm 1} \left(\frac{1}{2}\right)^{|i_1|+|j_1|+2}\omega_{i+i_1,j+j_1}.
\end{equation*}
Utilizing the $2$nd-order central difference scheme to discretize the mesh governing equations \eqref{eq:Mesh_Control} combined with the Jacobi iteration method gives
\begin{equation}
  \begin{aligned}\label{eq:JacobiIte}
    &\left[\left(\omega_{{i,j}}+\omega_{i+1,j}\right)\left(\bm{x}_{i+1,j}^{[\nu]}-\bm{x}_{{i,j}}^{[\nu+1]}\right)-\left(\omega_{{i,j}}+\omega_{i-1,j}\right)\left(\bm{x}_{{i,j}}^{[\nu+1]}-\bm{x}_{i-1,j}^{[\nu]}\right)\right]/\Delta \xi_1^{2}\\
    &+ \left[\left(\omega_{{i,j}}+\omega_{i,j+1}\right)\left(\bm{x}_{i,j+1}^{[\nu]}-\bm{x}_{{i,j}}^{[\nu+1]}\right)-\left(\omega_{{i,j}}+\omega_{i,j-1}\right)\left(\bm{x}_{{i,j}}^{[\nu+1]}-\bm{x}_{i,j-1}^{[\nu]}\right)
    \right]/\Delta \xi_2^{2}\\
    &=~0, ~\nu=0,1, \cdots, \mu-1,
  \end{aligned}
\end{equation}
where the initial mesh in the iterations $\bm{x}_{i,j}^{[0]}:=\bm{x}_{{i,j}}^n
$ is chosen as the mesh at $t^n$,
and the monitor function $\omega$ is computed based on the solution at $t^n$.
Once the grid $\left\{\bm{x}_{i,j}^{[\mu]}\right\}$ is obtained, the final adaptive mesh is given by
\begin{equation*}
  \bm{x}_{{i,j}}^{n+1}:=\bm{x}_{{i,j}}^n+\Delta_\tau\left(\delta_\tau \bm{ x}\right)_{i,j}^n,~\left(\delta_\tau \bm{x}\right)_{i,j}^n:=\bm{x}_{{i,j}}^{[\mu]}- \bm{x}_{{i,j}}^n,
\end{equation*}
with the parameter $\Delta_{\tau}$ to control the mesh movement
\begin{equation*}
  \Delta_\tau \leqslant \begin{cases}-\frac{1}{2\left(\delta_\tau x_1\right)_{i,j}^n}\left[\left(x_1\right)_ {{i,j}}^n-\left(x_1\right)_{i-1,j}^n\right], ~\left(\delta_\tau x_1\right)_{ {i,j}}<0, \\ +\frac{1}{2\left(\delta_\tau x_1\right)_{i,j}^n}\left[\left(x_1\right)_ {i+1,j}^n-\left(x_1\right)_{{i,j}}^n\right], ~\left(\delta_\tau x_1\right)_{ {i,j}}>0,\\
    -\frac{1}{2\left(\delta_\tau x_2\right)_{i,j}^n}\left[\left(x_2\right)_ {{i,j}}^n-\left(x_2\right)_{i,j-1}^n\right], ~\left(\delta_\tau x_2\right)_{ {i,j}}<0, \\ +\frac{1}{2\left(\delta_\tau x_2\right)_{i,j}^n}\left[\left(x_2\right)_ {i,j+1}^n-\left(x_2\right)_{{i,j}}^n\right], ~\left(\delta_\tau x_2\right)_{ {i,j}}>0.
  \end{cases}
\end{equation*}
Finally, the mesh velocities for the next time step are
\begin{equation*}
  \dot{\bm{x}}_{{i,j}}^n:=\Delta_\tau\left(\delta_\tau \bm{x}\right)_{i,j}^n / \Delta t^n,
\end{equation*}
where $\Delta t^{n}$ is the time stepsize given in \eqref{eq:dt}.


